Progressive and Aligned Pose Attention Transfer for Person Image Generation

This paper proposes a new generative adversarial network for pose transfer, i.e., transferring the pose of a given person to a target pose. We design a progressive generator which comprises a sequence of transfer blocks. Each block performs an intermediate transfer step by modeling the relationship between the condition and the target poses with attention mechanism. Two types of blocks are introduced, namely Pose-Attentional Transfer Block (PATB) and Aligned Pose-Attentional Transfer Bloc ~(APATB). Compared with previous works, our model generates more photorealistic person images that retain better appearance consistency and shape consistency compared with input images. We verify the efficacy of the model on the Market-1501 and DeepFashion datasets, using quantitative and qualitative measures. Furthermore, we show that our method can be used for data augmentation for the person re-identification task, alleviating the issue of data insufficiency. Code and pretrained models are available at https://github.com/tengteng95/Pose-Transfer.git.

==> 3method.tex <==
\section{Model}

% \subsection{Network Architecture}
\label{sec:network_architecture}
We begin with a few notations. $\left\{ P_{i}^{j}\right\}_{i=1\dots N_{j}}^{j=1\dots M}$
denotes the set of person images in a dataset, where $j$ is person index, $i$ is the image index of person $j$. $M$ is the number of persons, $N_j$ is the number of images of person $j$. 
$S_{i}^{j}$ is the corresponding keypoint-based representation of $P_{i}^{j}$, which consists of a 18-channel heat map that encodes the locations of 18 joints
of a human body. 
% In our work, the poses are estimated from images
% by a pose estimator. 
% For fair comparison, 
We adopt the Human Pose Estimator (HPE) \cite{HPE} used by \cite{poseguided,Disentangled,DeformableGAN} to estimate the 18 joints for fair comparison. During training, the model requires condition and target image $(P_c, P_t)$ and their corresponding condition and target pose heat map $(S_c,S_t)$. The generator outputs a person image, which is challenged by the discriminators for its realness.

% The following describes each in detail.

%Different from conventional generative adversarial network framework which consists of one generator and one discriminator, the proposed method comprises one generator and two discriminators. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Pose Morphing Sequence Generation}
% To alleviate the great challenge induced by large pose variations, we propose a pose morphing module to automatically generate pose morphing sequence from the condition pose $S_c$ to the target one $S_t$. The pose morphing sequence explicitly determines the generation process which learns to transfer the person image under $S_c$ to that under $S_t$ step by step. Each step is responsible for the generation process of two adjacent poses $S_i$ and $S_{i+1}$, which fall on a local manifold. In this way, the complex transfer process for two very different poses can be divided into several easier sub-process for poses with small changes.

% However, it is hard to design such a module to generate the pose morphing sequences. On the one hand, collecting a dataset with annotations of the morphing pose sequence between two poses is time-consuming. On the other hand, the morphing sequence from one pose to another is not unique. To overcome these limitations, we design a pose morphing module which can output a determined morphing pose sequence by interpolation in a unsupervised manner. Fig.~\ref{} illustrates the  architecture of our pose morphing module, which consists of a encoder and a decoder. Given a pose $S$, the encoder maps it to a latent code in the pose manifold. Accordingly, the decoder takes a latent code as input and recovers the corresponding pose. The overall module is very light-weighted, but surprisingly works well. Concretely, both of the encoder and the decoder comprise of only three fully connected layers. We add a leaky ReLU activation function after each fully connected layer except for the last one in the decoder part. In the training phase, we adopt the L2 loss to optimize the pose morphing module, which is formulate as follows:
% \begin{equation}
%     L_{PM} = (D(E(S))-S)^2
% \end{equation}
% where $S$ represents the input pose, D and E represents the encoder and the decoder respectively.
% In the testing phase, we can obtain the latent codes for the condition pose and the target pose, which are denoted as $E(S_c)$ and $E(S_t)$ respectively. We generate the latent codes of morphing pose sequence by interpolating $E(S_c)$ and $E(S_t)$. Then we use the decoder to recover the morphing pose sequence based on the interpolated latent codes.

% \subsection{Generator}
Fig.~\ref{fig:Generator} shows the architecture of the generator, which requires the inputs of the condition image $P_c$, the condition pose $S_c$ and the target pose $S_t$. The main aim of the generator is to transfer the pose of the person in the condition image $P_c$ from condition pose $S_c$ to target pose $S_t$, thus generates realistic-looking person image $P_g$. In general, our generator consists of two encoders, a pose transfer network, and a decoder, which are detailed in the following.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Encoders}
We employ two encoders in our generator: one encoder, called \emph{Appearance Encoder}, denoted as $E_A$, is used to encode the condition image to an image code; the other encoder, named \emph{Shape Encoder}, denoted as $E_S$, is used to map the condition pose $S_c$ and the target one $S_t$ to corresponding pose codes. In our setting, each encoder is comprised of one $7 \times 7$ convolution and two $3 \times 3$ convolutions with stride 2. We add a BatchNorm layer and a ReLU activation function after each convolution layer. Such a lighted-weighted network encodes valid features and saves the computation overhead for the following pose transfer process.

% for extracting feature representations with richer semantic information but lower spatial resolution for images and poses respectively. On the input side, the condition image is encoded into an image code by an image encoder $E_A$; The condition pose $S_c$ and the target one $S_t$ are encoded into the pose code by a pose encoder $E_S$. In our setting, each encoder is comprised of one $7 \times 7$ convolution and two $3 \times 3$ convolutions with stride 2. We add a BatchNorm layer and a ReLU activation function after each convolution layer. Such a lighted-weighted network encodes valid features and saves the computation overhead for the following pose transfer process.

% On the input side, the condition image is encoded by an image encoder; The condition pose $S_c$ and the target one $S_t$ are encoded by a pose encoder. 

% On the input side, the condition image is encoded by an image encoder; All the poses in the pose morphing sequence from condition pose $S_c$ to the target one $S_t$ are encoded by a pose encoder. The encoded pose morphing sequence provides explicit guidance information of how to transfer person under $S_c$ to $S_t$ gradually step by step.

\subsection{Pose Transfer Network}
The core of our generator is the Pose Transfer Network. This network takes inputs the image code and pose code as inputs and then learns to transfer the person image under condition pose $S_c$ to the target pose $S_t$. The pose transfer, at a basic level, is about moving patches from
the locations induced by the condition pose to the locations induced by the target pose. In this sense, the pose guides the transfer process by hinting \emph{where to sample condition patches} and \emph{where to put target patches}. However, large pose variations brings great challenge for this \textit{sample-and-put} operation. To address the issue, we design a progressive pose transfer network which consists of a series of pose transfer blocks. 

The design of the pose transfer block is crucial for the Pose Transfer Network. In our conference version, we propose a Pose Attentional Transfer Network~(PATN) with multiple Pose Attentional Transfer Blocks~(PATB). In the following, we first present a review of PATN and PATB. Then we present a new solution named Pose Morphing Transfer Network~(PMTN) which achieves the progressive transfer process with several Pose Morphing Transfer Blocks~(PMTB) guided by a pose morphing sequence.

% In our network, such hints can realized by the
% \emph{attention mask} denoted as $M_t$, which are values between 0 and 1 indicating the importance of every element in the image code. How to obtain a effective attention mask is crucial for the pose transfer process. In our original conference paper, we propose the Pose Attentional Transfer Block~(PATB) which implicitly learns the attention mask by enhancing or suppressing some spatial postions feature representation
% To alleviate the great challenge induced by large pose variations, we propose the pose transfer network which transfers the person image under condition pose $S_c$ to the target pose $S_t$ in a progressive manner. is The pose transfer network works as the core part of our generator since it involves with the transfer process for both shape and appearance.  

% The pose transfer, at a basic level, is about moving patches from
% the locations induced by the condition pose to the locations induced by the target pose. In this sense, the pose guides the
% transfer by hinting \emph{where to sample condition patches }and \emph{where to put target patches}. 
% In our network, such hints can realized by the
% \emph{attention mask} denoted as $M_t$, which are values between 0 and 1 indicating the importance of every element in the image code. How to obtain a effective attention mask is crucial for the pose transfer process. In our original conference paper, we propose the Pose Attentional Transfer Block~(PATB) which implicitly learns the attention mask by enhancing or suppressing some spatial postions feature representation

% To alleviate the great challenge induced by large pose variations, we propose a pose morphing module to automatically generate pose morphing sequence from the condition pose $S_c$ to the target one $S_t$. The pose morphing sequence explicitly determines the generation process which learns to transfer the person image under $S_c$ to that under $S_t$ step by step. Each step is responsible for the generation process of two adjacent poses $S_i$ and $S_{i+1}$, which fall on a local manifold. In this way, the complex transfer process for two very different poses can be divided into several easier sub-process for poses with small changes.

% In the following, we first review the Pose-Attentional Transfer Network~(PATN) proposed in our original conference version. Then we present a new Pose Morphing Transfer Network~(PMTN) which achieves the transfer process with guidance of a sequence of morphing poses.

\subsubsection{Pose-Attentional Transfer Network}


\begin{figure}
		% \vspace{-0.5cm}
		\centering
		\includegraphics[width=0.48\textwidth]{imgs/PATB.pdf}
		\caption{Architecture of our PATB.\label{fig:PMTB}}
	\end{figure}

Pose-Attentional Transfer Network (PATN) consists of several cascaded Pose-Attentional Transfer Blocks (PATBs). Starting from the initial image code $F_{0}^{P}$ and joint pose code $F_{0}^{S}$, PATN progressively updates these two codes through the sequence of PATBs. At the output, the final image code $F_T^P$ are taken to decode the output image, while the final pose code $F_T^S$ is discarded.

All PATBs have identical structure. A PATB carries out one
step of update. Consider the $t$-th block, whose inputs are $F_{t-1}^{P}$
and $F_{t-1}^{S}$. As depicted in Fig.~\ref{fig:Generator}, the block comprises two pathways, called \emph{image pathway}
and \emph{pose pathway} respectively. With interactions, the two
pathways update $F_{t-1}^{P}$ and $F_{t-1}^{S}$ to $F_{t}^{P}$
and $F_{t}^{S}$, respectively. 
The interaction is mainly dependent on the attention mechanism. The pose pathway produces element-wise pose attention mask $M_{t}$ for the image pathway by feeding the pose code $F_{t-1}^{S}$ through some convolutions $\text{conv}_{S}$ and a Sigmoid layer that maps the values of the attention mask to the interval of $[0, 1]$. The image code also goes through several convolutions $\text{conv}_{P}$ and the resulted feature map is multiplied with the attention mask in an element-wise manner. This multiplication intuitively retains important features and suppress irrelevant features. \textcolor{red}{The output of the element-wise product is added by
FP , constituting a residual connection [9]. The residual t−1
connection helps preserve the original image code, which is critical for the pose transfer. Having residual connection also eases the training as observed in [9], particularly when there are many PATBs.} Mathematically, the image code $F_{t}^{P}$ is updated by:
\begin{equation}
F_{t}^{P}=M_{t}\odot\text{conv}_{P}\left(F_{t-1}^{P}\right)+F_{t-1}^{P}.
\end{equation}
As the image code gets updated through the PATBs, the pose code should also be updated to synchronize the change:
\begin{equation}
F_{t}^{S}=\mathrm{conv}_{S}\left(F_{t-1}^{S}\right)\Vert F_{t}^{P}.
\end{equation}



% In the following, we describe the detailed update process in three
% parts and justify their designs.

% \vspace{1ex}\noindent\textbf{Pose Attention Masks.} As mentioned above, the pose guides the
% transfer process by hinting \emph{where to sample condition patches }and \emph{where to put target patches}. In our PATB, such hints are realized by the
% \emph{attention mask} denoted as $M_t$, which are values between 0 and 1 indicating the importance of every element in the image code.

% The attention masks $M_t$ are computed from the pose code $F_{t-1}^{S}$, which incorporates
% both the condition and the target pose. The pose code $F_{t-1}^{S}$ firstly goes through
% two convolutional layers (with a normalization layer \cite{batchnorm,instancenorm} and ReLU \cite{ReLU} in between), before
% being mapped to the range of $(0,1)$ by an element-wise $\mathrm{sigmoid}$
% function. Mathematically:
% \begin{equation}
% \label{w_t}
% M_{t}=\sigma\left(\mathrm{conv}_{S}\left(F_{t-1}^{S}\right)\right).
% \end{equation} 

% % \vspace{-2mm}
% \vspace{1ex}\noindent\textbf{Image Code Update.}
% Having computed $M_{t}$, the image code $F_{t}^{P}$ is updated by:
% \begin{equation}
% F_{t}^{P}=M_{t}\odot\text{conv}_{P}\left(F_{t-1}^{P}\right)+F_{t-1}^{P} ,
% \end{equation}
% where $\odot$ denotes element-wise product. By multiplying the transformed
% image codes with the attention masks $M_t$, image code $F_{t}^{P}$ at certain locations
% are either preserved or suppressed. The output of the element-wise product is added by $F_{t-1}^{P}$, constituting a \emph{residual connection} \cite{resnet}. 
% The residual connection
% helps preserve the original image code, which is critical for the
% pose transfer. Having residual connection also eases the training as observed in \cite{resnet},
% particularly when there are many PATBs.

% \vspace{1ex}\noindent\textbf{Pose Code Update.}
% As the image code gets updated through the PATBs, the pose code
% should also be updated to synchronize the change, \emph{i.e.} update
% where to sample and put patches given the new image code. Therefore,
% the pose code update should incorporate the new image code.

% Specifically, the previous pose code $F_{t-1}^{S}$ firstly goes through two convolutional layers (with a normalization layer and ReLU in between). Note when $t>1$, the first convolutional layer will reduce the feature map depth to half, making the feature map depths of subsequent layers in the pose pathway equal to those in the image pathway.
% Then, the transformed code
% is mixed with the updated image code by concatenation. Mathematically,
% the update is performed by
% \begin{equation}
% F_{t}^{S}=\mathrm{conv}_{S}\left(F_{t-1}^{S}\right)\Vert F_{t}^{P} ,
% \end{equation}
% where $\Vert$ denotes the concatenation of two maps along depth
% axis.



\subsubsection{Pose Morphing Transfer Network}
\label{PMTN}

\vspace{1ex}\textbf{Overview.}~With thorough investigation about PATN, we found two issues that may limit the performance of the pose transfer task. First, there is no explicit guidance about how to transfer the pose step by step. Hence, the behaviour of the PATBs is unpredictable and lacks interpretability. Second, PATB learns to enhance or suppress related area in the image code through an attention mask. This operation evaluates the importance of each spatial position separately, but ignores the explicit alignment between the condition pose and the target pose. Hence, it brings difficulty in conducting the \textit{sample-and-put} operation~(\textit{i.e.}, where to sample and where to put), leading to sub-optimal performance.
% With thorough investigation about PATN, we found two issues that may limit performance in performing the pose transfer task. First, PATN \emph{implicitly} splits the whole transfer process into several progressive stages where each stage is conducted by a PATB. This setting gives the model sufficient capacity to adjust the transfer process automatically but makes the whole process less explainable. Second, we previously leverage pose features to produce attention mask which is multiplied to the appearance feature in order to suppress or enhance specific feature representations. This pixel-wise operation has the inherit difficulty to move a feature to somewhere else in the image, which is critical to maximumly preserve appearance details.

To alleviate these two issues, we devise a new Pose Morphing Transfer Network~(PMTN), which comprises of several cascaded Pose Morphing Transfer Block (PMTB). PMTN is different from PATN in two folds. First, PMTN takes as input a pose sequence, which consists of several intermediate pose frames starting from the condition pose $S_c$ to the target pose $S_t$, while PATN only takes in the $S_c$ and the $S_t$. This pose sequence provides two adjacent poses as the condition pose and target pose for each PMTB, which is then responsible for a local pose transfer in the whole process. Considering that adjacent poses in the sequence usually share less variation, this design considerably alleviates the transfer difficulty caused by the large variation between $S_c$ and $S_t$. 

% determined and explicit guidance to each PMTB in order to conduct the transfer process step by step. Each PMTB is responsible for a sub-process of pose transfer between two adjacent poses of the sequence. 


Second, we update our attention mechanism in a more reasonable way to preserve more local details. In PATB, it's done by feeding the combined pose features of the condition and target pose to a residual block to produce the attention mask directly. However, this method ignores the spatial correspondence of the condition and target pose, which is helpful to smoothly move the features to correct positions. In our updated attention mechanism of PMTB, we calculate the correspondence of the two adjacent poses and then aggregate the features of the image code according to this location correspondence. This new attention mechanism enables PMTB to \emph{sample-and-put} features directly and smoothly, thus it largely helps preserve local details.

% As discussed previously, pose transfer is about moving patches from the condition pose to places indicated by the target pose. Therefore, 



% a new solution for generating the attention mask, which explicitly align the condition pose and the target pose. 

% To alleviate these two issues, we devise a new Pose Morphing Transfer Network~(PMTN), which comprises of several cascaded Pose Morphing Transfer Block (PMTB). PMTN is different from PATN in two folds. First, PMTN achieves the transfer process with determined and explicit guidance of the pose morphing sequence, different from PATN which implicitly infer the transfer path. Every PMTB is responsible for pose transfer between adjacent poses in the sequence which falls in a local pose manifold. Second, each PMTB receives the previous pose code in the last step and the next pose code to transfer while PATB implicitly update the combined condition and target poses step by step.

% Accordingly, we design a pose morphing model to adaptively generate the pose morphing sequence from given condition pose to the target pose. PMTN takes the pose sequence as inputs and gradually achieve the transfer process. 


In the following, we will illustrate the details and the design of the pose morphing transfer block and then present the details of how to obtain the pose morphing sequence. 

% we first present details of how to obtain the pose morphing sequence. Then we illustrate the details and the design of the pose morphing transfer block.

\label{sec:PMTN}

\vspace{1ex}\noindent\textbf{Pose Morphing Transfer Block.} The Pose Morphing Transfer Block~(PMTB) is the core part of our pose morphing transfer network. All PMTBs have identical structure. Each PMTB carries out one step of update for two adjacent poses in the pose morphing sequence. Consider the t-th block whose inputs are the image code $F_{t-1}^{P}$, and two adjacent pose codes in the pose morphing sequence, \textit{i.e.}, $F_{t-1}^{S}$ and $F_{t}^{S}$. PMTB learns to align the two pose codes and updates the image code $F_{t-1}^{P}$ to $F_{t}^{P}$ accordingly to produce image semantic features under $F_{t}^{P}$.

How to effectively align two pose codes is of great importance for the transfer process, since it explicitly provides the guidance about where to sample and where to put. A straight solution is to calculate the similarity between all pairs of spatial positions from the pose codes. Fig.~\ref{fig:PMTB} illustrates the structure of our PMTB. Consider two adjacent pose codes $F_{t-1}^{S}$ and $F_{t}^{S}$ in the pose morphing sequence, each of which is in the shape of $C\times H \times W$, where $C$, $H$, $W$ denote the channel dimension, the height, and the width, respectively. We first feed the pose codes $F_{t-1}^{S}$ and $F_{t}^{S}$ to a $1\times1$ convolution layer to reduce their channel dimension. Then we calculate the similarity matrix $M_t$ of these two pose codes in a matrix inner production manner, which can be formulated as follows:
\begin{equation}
M_t = \mathrm{conv}_{\theta}(F_{t}^{S}) \times \mathrm{conv}_{\phi}(F_{t-1}^{S})^T
\end{equation}
where $\mathrm{conv}_{\theta}(\cdot)$ and $\mathrm{conv}_{\phi}(\cdot)$ denote the $1\times 1$ convolution layer, $\times$ represents the matrix inner production. The similarity matrix $M_t$ is in the shape of $(HW) \times (HW)$, indicating the similarity of all the pairs of the spatial positions. We apply the softmax function to $M_t$ so that the sum of each row and each column is equal to 1. 

The pose attention mask $M_t$ provide explicit guidance about where to sample the condition patch for each location of the current image code. Hence, we can update current image code through a matrix inner production operation between $M_t$ and $F_{t-1}^{P}$, which can be written as
\begin{equation}
F_{t}^{P}=M_{t} \times F_{t-1}^T ,
\end{equation}
In this way, the PMTB learns to sample and put the condition patch to the target area indicated by the attention masks $M_t$. We further update $F_{t}^{P}$ with a combination of $F_{t}^{P}$ and $F_{t-1}^{P}$ to avoid information loss and to benefit the gradient backpropagation. 

Note that the operations above only involves a few learnable parameters in the $1\times1$ convolution layers. To increase the model capacity and better leverage the combination of previous and updated image codes, we introduce a extra residual block~\cite{resnet} which comprise of a $3\times3$ conolutional layer, a batch normalization layer and a ReLU activation function layer. 

\vspace{1ex}\noindent\textbf{Pose Morphing Sequence Generation.} To alleviate the great challenge induced by large pose variations, we propose a pose morphing module to automatically generate a series of pose frames from the condition pose $S_c$ to the target one $S_t$. The pose morphing sequence explicitly determines the generation process, that is, how to transfer the person image under $S_c$ to that under $S_t$ step by step. Each step is responsible for a local pose transfer process for two adjacent poses $S_i$ and $S_{i+1}$. In this way, the complex transfer process for two very different poses can be divided into several easier sub-process for poses with less variation.

However, it is hard to design such a module to generate the pose morphing sequences. On the one hand, collecting a dataset with annotations of the morphing pose sequence between two poses is expensive. On the other hand, the morphing sequence from one pose to another is not unique. To overcome these limitations, we design a pose morphing module which can output a determined morphing pose sequence by linear interpolation of the poses from the latent space in a unsupervised manner. Our pose morphing module consists of a encoder $E_P$ and a decoder $D_P$. Given a pose $S$, the encoder maps it to a latent code. Accordingly, the decoder learns to recover the corresponding pose from a given latent code. The overall module is very light-weighted, but surprisingly works well. Concretely, both of the encoder and the decoder comprise of only three fully connected layers. We add a leaky ReLU activation function after each fully connected layer except for the last one in the decoder part. 

Through the encoder, we can obtain the latent codes for the condition pose and the target pose, which are denoted as $\upsilon(S_c)$ and $\upsilon(S_t)$ respectively. And we can generate a series of middle latent codes using a linear interpolation of $\upsilon(S_c)$ and $\upsilon(S_t)$, from which we can recover the corresponding poses and obtain the pose morphing sequence. We formularize this process as follows:
% \begin{equation}
%     \mathcal{S}_i = (1-\frac{i}{\mathcal{N}}\mathcal{S}_0) + \frac{i}{\mathcal{N}}\mathcal{S}_{\mathcal{N}-1},
% \end{equation}
% where $\mathcal{S}_i$ denotes the i-th pose in the pose morphing sequence, $\mathcal{N}$ represents the length of the pose morphing sequence. $\mathcal{S}_0$ and $\mathcal{S}_(\mathcal{N}-1)$ are the first and the last pose in the pose morphing sequence.
% \begin{equation}
%     S_i = D_P((1-\frac{i}{\mathcal{N}})S_0 + \frac{i}{\mathcal{N}}S_{\mathcal{N}-1}),
% \end{equation}
\begin{equation}
    \upsilon(S_i) = \varphi((1-\frac{i}{\mathcal{N}})\upsilon(S_c)+ \frac{i}{\mathcal{N}}\upsilon(S_t)),
\end{equation}
where $\mathcal{N}$ represents the length of the pose morphing sequence. $\varphi$ denotes the function of the decoder. $S_0$ and $S_{(\mathcal{N}-1)}$ are the latent codes for the first pose $\upsilon(S_c)$ and the last pose $\upsilon(S_t)$ in the pose morphing sequence.
% where $S_i$ denotes the i-th pose in the pose morphing sequence, $\mathcal{N}$ represents the length of the pose morphing sequence. $S_0$ and $S_{(\mathcal{N}-1)}$ are the first and the last pose in the pose morphing sequence.

In the training phase, we adopt a reconstruction loss to ensure the consistency between the recovered pose from the decoder and the input pose.  Besides, we introduce a extra regularization term to smooth the generated pose morphing sequence and to avoid large variation between two adjacent poses. The total optimization function is formulated as follows:

\begin{equation}
    L_{PM} = \underbrace{(\varphi(\upsilon(S))-S)^2}_{reconstruction \ loss} + \underbrace{\sum_{i=2}^{\mathcal{N}-1}(S_{i-1} +  S_{i+1} - 2S_{i})}_{regularization \ loss}
\end{equation}
where $L_PM$ represent the total loss for our pose morphing module, respectively. It worth noting that we simply ignore those unobserved joints and do not calculate their losses. 
% \begin{equation}
%     L_{PM\_L2} = (D_P(E_P(S))-S)^2 ,
% \end{equation}


% \begin{equation}
%     L_{rec} = (\varphi(\upsilon(S))-S)^2 ,
% \end{equation}

% \begin{equation}
%     L_{reg} = \sum_{i=1}^{\mathcal{N}-1}(S_{i-1} +  S_{i+1} - 2S_{i}) ,
% \end{equation}

% \begin{equation}
%     L_{PM} = L_{rec} + L_{reg} ,
% \end{equation}
% where $L_{rec}$, $L_{reg}$, and $L_PM$ represent the reconstruction loss, the regularization loss, and the total loss for our pose morphing module, respectively. It worth noting that we simply ignore those unobserved joints and do not calculate their losses. 
 



% The residual block helps preserve the original image code, which is critical for the pose transfer. Having residual connection also eases the training as observed in \cite{resnet}, particularly when there are many PATBs.

% At the core of the generator is the \emph{Pose Morphing Transfer Network} (PMTN), consisting of several cascaded Pose-Morphing Transfer Blocks (PMTBs). PMTN takes the initial image code $F_{0}^{P}$ and a sequence of pose code $F_{i}^{S}$~(i=0,1,...,T) as inputs, and progressively transfer current pose to the next one through a corresponding sequence of PMTBs. Finally, we keep the last image code $F_T^P$ which has already been transferred to the target pose $S_t$ while discard the final pose code $F_T^S$.

% At the core of the generator is the \emph{Pose Morphing Transfer Network} (PMTN), consisting of several cascaded Pose-Morphing Transfer Blocks (PMTBs).
% Starting from the initial image code $F_{0}^{P}$ and joint pose code $F_{0}^{S}$, PATN progressively updates these two codes through the sequence of PATBs. At the output, the final image code $F_T^P$ are taken to decode the output image, while the final pose code $F_T^S$ is discarded.

% All PMTBs have identical structure. A PMTB carries out one
% step of update for two adjacent poses in the pose morphing sequence. As depicted in Fig.~\ref{fig:Generator}, each block comprises two pathways called \emph{image pathway}
% and \emph{pose pathway} respectively. Consider the $t-th$ block whose inputs are the image code $F_{t-1}^{P}$ and the pose code $F_{t-1}^{S}$ from the last step, as well as current pose code $F_{t}^{S}$. PMTB learns to align the two pose codes and updates the image code $F_{t-1}^{P}$ to $F_{t}^{P}$ accordingly to produce image semantic features under $F_{t}^{P}$.

% All PATBs have identical structure. A PATB carries out one
% step of update. Consider the $t$-th block, whose inputs are $F_{t-1}^{P}$
% and $F_{t-1}^{S}$. As depicted in Fig.~\ref{fig:Generator}, the block comprises two pathways, called \emph{image pathway}
% and \emph{pose pathway} respectively. With interactions, the two
% pathways update $F_{t-1}^{P}$ and $F_{t-1}^{S}$ to $F_{t}^{P}$
% and $F_{t}^{S}$, respectively.

% In the following, we present the detailed update process in our PMTB.

\begin{figure}
		% \vspace{-0.5cm}
		\centering
		\includegraphics[width=0.48\textwidth]{imgs/PMTB.pdf}
		\caption{Architecture of our PMTB.\label{fig:PMTB}}
	\end{figure}

% \vspace{1ex}\noindent\textbf{Pose Attention Masks.}
% The pose transfer, at a basic level, is about moving patches from
% the locations induced by the condition pose to the locations induced by the target pose. In this sense, the pose guides the
% transfer by hinting \emph{where to sample condition patches }and \emph{where to put target patches}. In our network, such hints are realized by the
% \emph{attention mask} denoted as $M_t$, which are values between 0 and 1 indicating the importance of every element in the image code.

% How to effectively align the joints between two pose codes is the core part of obtaining a reasonable pose attention mask. A straight solution is to calculate the similarity between the pose codes. Now we have two adjacent pose codes $F_{t-1}^{S}$ and $F_{t}^{S}$ in the pose morphing sequence. Considering that evaluating the similarity of all the positions pairs between them are computationally intensive and time-consuming, we sample a subset of crucial spatial positions from $F_{t-1}^{S}$ and evaluate similarity matrix between $F_{t}^{S}$ and the sampled positions, which is similar to ANN~\cite{}. Concretely, we first feed the pose code $F_{t-1}^{S}$ and $F_{t}^{S}$ to a $1\times1$ convolution layer to reduce their channel dimension. Then we employ a spatial pyramid pooling module, which consists of four average pooling layers with the kernel size of \{$H\times W$, $\frac{H}{3}\times\frac{W}{3}$, $\frac{H}{6}\times\frac{W}{6}$, $\frac{H}{8}\times\frac{W}{8}$\}. In other words, we obtain four feature maps in the shape of \{ $1\times1$, $3\times 3$, $6\times6$, $8\times8$ \}, respectively. We flatten them and concatenate them together to obtain the distilled representation of the pose code $F_{t-1}^{S}$. Then the similarity matrix can be calculated as follows:
% \begin{equation}
% M_t = F_{t}^{S} \times F_{t-1}^{S}
% \end{equation}
% where $\times$ represents the matrix inner production.


% \vspace{-2mm}
% \vspace{1ex}\noindent\textbf{Image Code Update.} The pose attention mask $M_t$ provide explicit guidance about where to sample the condition patch for each location of the current image code. Hence, we generate current image code through a matrix inner production operation of $M_t$ and $F_{t-1}^{P}$. Then we employ a residual block\ref{} which comprise of a $3\times3$ conolutional layer, a batch normalization layer and a ReLU activation function layer,

% Having computed $M_{t}$, the image code $F_{t}^{P}$ is updated by:
% \begin{equation}
% F_{t}^{P}=M_{t}\odot\text{conv}_{P}\left(F_{t-1}^{P}\right)+F_{t-1}^{P} ,
% \end{equation}
% where $\odot$ denotes element-wise product. By multiplying the transformed
% image codes with the attention masks $M_t$, image code $F_{t}^{P}$ at certain locations
% are either preserved or suppressed. The output of the element-wise product is added by $F_{t-1}^{P}$, constituting a \emph{residual connection} \cite{resnet}. 


% Mathematically:
% \begin{equation}
% F_{t}^{P}=F_t^W+F_{t-1}^{P}
% \end{equation}






% \subsubsection{Pose-Attentional Transfer Network}

% At the core of the generator is the \emph{Pose-Attentional Transfer Network} (PATN), consisting of several cascaded Pose-Attentional Transfer Blocks (PATBs). Starting from the initial image code $F_{0}^{P}$ and joint pose code $F_{0}^{S}$, PATN progressively updates these two codes through the sequence of PATBs. At the output, the final image code $F_T^P$ are taken to decode the output image, while the final pose code $F_T^S$ is discarded.

% All PATBs have identical structure. A PATB carries out one
% step of update. Consider the $t$-th block, whose inputs are $F_{t-1}^{P}$
% and $F_{t-1}^{S}$. As depicted in Fig.~\ref{fig:Generator}, the block comprises two pathways, called \emph{image pathway}
% and \emph{pose pathway} respectively. With interactions, the two
% pathways update $F_{t-1}^{P}$ and $F_{t-1}^{S}$ to $F_{t}^{P}$
% and $F_{t}^{S}$, respectively.

% In the following, we describe the detailed update process in three
% parts and justify their designs.

% \vspace{1ex}\noindent\textbf{Pose Attention Masks.}
% The pose transfer, at a basic level, is about moving patches from
% the locations induced by the condition pose to the locations induced by the target pose. In this sense, the pose guides the
% transfer by hinting \emph{where to sample condition patches }and \emph{where to put target patches}. In our network, such hints are realized by the
% \emph{attention mask} denoted as $M_t$, which are values between 0 and 1 indicating the importance of every element in the image code.

% The attention masks $M_t$ are computed from the pose code $F_{t-1}^{S}$, which incorporates
% both the condition and the target pose. The pose code $F_{t-1}^{S}$ firstly goes through
% two convolutional layers (with a normalization layer \cite{batchnorm,instancenorm} and ReLU \cite{ReLU} in between), before
% being mapped to the range of $(0,1)$ by an element-wise $\mathrm{sigmoid}$
% function. Mathematically:
% \begin{equation}
% \label{w_t}
% M_{t}=\sigma\left(\mathrm{conv}_{S}\left(F_{t-1}^{S}\right)\right).
% \end{equation} 

% % \vspace{-2mm}
% \vspace{1ex}\noindent\textbf{Image Code Update.}
% Having computed $M_{t}$, the image code $F_{t}^{P}$ is updated by:
% \begin{equation}
% F_{t}^{P}=M_{t}\odot\text{conv}_{P}\left(F_{t-1}^{P}\right)+F_{t-1}^{P} ,
% \end{equation}
% where $\odot$ denotes element-wise product. By multiplying the transformed
% image codes with the attention masks $M_t$, image code $F_{t}^{P}$ at certain locations
% are either preserved or suppressed. The output of the element-wise product is added by $F_{t-1}^{P}$, constituting a \emph{residual connection} \cite{resnet}. 
% % Mathematically:
% % \begin{equation}
% % F_{t}^{P}=F_t^W+F_{t-1}^{P}
% % \end{equation}
% The residual connection
% helps preserve the original image code, which is critical for the
% pose transfer. Having residual connection also eases the training as observed in \cite{resnet},
% particularly when there are many PATBs.

% \vspace{1ex}\noindent\textbf{Pose Code Update.}
% As the image code gets updated through the PATBs, the pose code
% should also be updated to synchronize the change, \emph{i.e.} update
% where to sample and put patches given the new image code. Therefore,
% the pose code update should incorporate the new image code.

% Specifically, the previous pose code $F_{t-1}^{S}$ firstly goes through two convolutional layers (with a normalization layer and ReLU in between). Note when $t>1$, the first convolutional layer will reduce the feature map depth to half, making the feature map depths of subsequent layers in the pose pathway equal to those in the image pathway.
% %Specifically, the previous pose code $F_{t-1}^{S}$ firstly goes through a depth-reduction convolutional layer to reduce half of the depth, making the feature map depths of subsequent layers in the pose pathway equal to those in the image pathway. Then another convolutional layer is followed (with a normalization layer and ReLU in between), to increase the capacity. 
% Then, the transformed code
% is mixed with the updated image code by concatenation. Mathematically,
% the update is performed by
% \begin{equation}
% F_{t}^{S}=\mathrm{conv}_{S}\left(F_{t-1}^{S}\right)\Vert F_{t}^{P} ,
% \end{equation}
% where $\Vert$ denotes the concatenation of two maps along depth
% axis.

\subsection{Decoder}
The updates in the pose transfer network result in the final image code $F_{T}^{P}$ and
the final pose code $F_{T}^{S}$. We take the image code and discard
the final pose code. Following the standard practice, the decoder recovers the image resolution and generates the transferred image $P_{g}$ from $F_{T}^{P}$ via several upsampling operations. In our setting, the decoder is adopted as a similar architecture to our encoder. Concretely, we adopt two bilinear upsamling layers and a $7\times7$ convolution layer followed by a tanh activation function. We add a residual block after each upsampling layer to enhance the capacity and smooth the feature representation.
% The updates in PATN result in the final image code $F_{T}^{P}$ and
% the final pose code $F_{T}^{S}$. We take the image code and discard
% the final pose code. Following the standard practice, the decoder generates
% the output image $P_{g}$ from $F_{T}^{P}$ via $N$ deconvolutional
% layers.

% \begin{figure}
% % \vspace{-0.5cm}
% \begin{centering}
% \includegraphics[width=0.5\textwidth]{Figures/Discriminators}
% \par\end{centering}
% \caption{Appearance discriminator and shape discriminator\label{fig:Discriminators}}
% \end{figure}

\subsection{Discriminators}

%The discriminator judges the realness of the generated image $P_{g}$ in order to improve the generation quality. During training, the discriminator is trained by the generated images and the real target images, along with their real/fake labels.

%A typical discriminator directly judges $P_{g}$ with a convolutional
%neural network. However, this ignores the context of the input poses
%and the condition image. To judge the quality of the pose transfer,
%the discriminator should not only judges how real $P_{g}$ looks,
%but also how likely $P_{g}$ contains the same person in $P_{c}$
%(\emph{appearance consistency}), and how well $P_{g}$ align with
%the target pose $S_{t}$ (\emph{shape consistency}).

%To judge the quality of the pose transfer, 
We design two discriminators called \emph{appearance discriminator} $D_{A}$ and \emph{shape discriminator} $D_{S}$, to judge how likely $P_{g}$ contains the same person in $P_{c}$ (\emph{appearance consistency}) and how well $P_{g}$ align with the target pose $S_{t}$ (\emph{shape consistency}).
%the discriminator should not only judges how real $P_{g}$ looks, but also how likely $P_{g}$ contains the same person in $P_{c}$ (\emph{appearance consistency}), and how well $P_{g}$ align with the target pose $S_{t}$ (\emph{shape consistency}). Based on the foregoing, we design two discriminators. The first one is called \emph{appearance discriminator} denoted as $D_{A}$, which judges $P_{g}$ conditioned on $P_{c}$. The second one is called \emph{shape discriminator} denoted as $D_{S}$, which judges $P_{g}$ conditioned on $S_{t}$. 
The two discriminators
have similar structures, where $P_{g}$ is concatenated with either
$P_{c}$ or $S_{t}$ along the depth axis, before being fed into a
CNN (convolutional neural network) for judgment. Their outputs are respectively $R^{A}$ and $R^{S}$,
\emph{i.e.} the appearance consistency score and the shape consistency
score. The scores are the probabilities output by the softmax layer
of a CNN. The final score $R$ is the production of the two scores: $R=R^{A}R^{S}$.

% One can easily imagine combining the two discriminators into one that is conditioned on both $P_{c}$ and $S_{t}$ to directly estimate $R$. However, we argue that the tasks carried out by the two discriminators have different, conflicting natures. The appearance discriminator judges whether two persons are identical, regardless of their poses. Such a discriminator should focus on the appearance consistency of local patches and disregard patch locations. Meanwhile, the shape discriminator judges how well the person align with the given target pose. This task focuses on the consistency of patch locations rather than appearance. Therefore, using separate networks for the two tasks reduces the conflict, leading to better performance in practice. This will be experimentally verified later.

% \vspace{-2mm}

%\subsubsection{Discriminator architecture}

% Since the birth of GAN, few works have discussed about the architecture of discriminator. Most works treat discriminator as a simple classification network by only integrating several convolutions. 
% Gulrajani \emph{et al.} \cite{WGAN-GP} firstly train a functional WGAN-GP network with residual blocks, showing the possibility to use more powerful architectures such as residual blocks in discriminators.  \cite{spectralnormalization}
% This reason can be attributed to the unstable training of GAN. To train a fully functional GAN network, we have to carefully balance the ability to avoid generator or discriminator overwhelms the other one at early training stages. Generally speaking, generator is weak when the training starts, so weakening discriminator will guarantee a stable training startup. 
As the training proceeds, we observe that a discriminator with low capacity becomes insufficient to differentiate real and fake data. 
%One may easily consider a more powerful discriminator might be helpful. 
Therefore, we build the discriminators by adding three residual blocks after two down-sampling convolutions to enhance their capability. 
%Different from vanilla PatchGAN discriminator \cite{pix2pix2017-cvpr}, no depth-reduction convolution is followed for the experimentally better results.
% This simple and fluent architecture called \emph{ResD} brings considerable performance improvements through experiments.


% spatial prediction may potentially reduce artifacts and is more robust than plane prediction. 
% Note that the number of down-sampling convolutions and residual blocks is up to the image size of the datasets. We recommend that the receptive field size should keep around \(\frac{1}{3}\) to \(\frac{1}{2}\) of the input image' size.

% Besides, we make several modifications to the residual blocks in our ResD. We omit all Dropout operations and we replace the typical ReLU function in residual blocks to leaky ReLU with the negative slope coefficient set to 0.2. 
% as many techniques \cite{improvedtrainingGAN,TowardsPrincipled,arjovsky2017wgan} are proposed to deal with the unstable training behavior of GAN, we believe strengthening discriminator will be beneficial to the whole training process.

% He et al. \cite{resnet} proposed a very effective model called ResNet to solve the training problems of very deep networks and achieved significant results in object classification and detection. The fundamental component of ResNet is a network architecture named residual block. Residual block is extensively useful to enlarge the capacity of a convolutional network model because even in the worst case, the convolutions inside a residual block are useless while the skip connection still contributes to the final results. Considering these advantages of residual block, we decide to integrate it to our discriminator architecture design.
% The idea is simple and empirical. As depicted in Fig.\ref{fig:model}, 

\subsection{Loss function for pose transfer}

\label{lossfunction}
	The full loss function is denoted as:
	\begin{equation}
	\mathcal{L}_{full}=\arg\underset{G}{\min}\, \underset{D}{\max}\, \alpha \mathcal{L}_{GAN} + \beta\mathcal{L}_{L1}+\gamma\mathcal{L}_{perL1},,
	% \mathbb{E}_{x\sim p(x)}
	\end{equation}
	where $\mathcal{L}_{GAN}$ denotes the adversarial loss, $\mathcal{L}_{L1}$ denotes the pixel-wise $L_1$ loss computed between the generated and target image and $\mathcal{L}_{L1}=\left \| P_{g}-P_t \right \|_1$ and $\mathcal{L}_{perL1}$ represents the perceptual loss widely used in the tasks of super-resolution \cite{SRGAN}, style transfer \cite{perceptualloss}, \emph{etc}. Note $\alpha, \beta, \gamma$ represents the weights of $\mathcal{L}_{GAN}$, $\mathcal{L}_{L1}$ and $\mathcal{L}_{perL1}$, respectively. We empirically find that perceptual loss is helpful to reduce pose distortion and make the produced images look more natural and smooth. This type of loss is also used in other pose transfer methods~\cite{vunet}. In formula, 
	\begin{small}
		\begin{equation}
		\mathcal{L}_{perL1}=\frac{1}{W_{\rho}H_{\rho }C_{\rho}} \sum_{x=1}^{W_{\rho }}\sum_{y=1}^{H_{\rho }}\sum_{z=1}^{C_{\rho }}\left \| \phi _{\rho }(P_{g})_{x,y,z}-\phi _{\rho }(P_t)_{x,y,z} \right \|_1,
		\end{equation}
	\end{small}where $\phi _{\rho }$ are the outputs of a layer, indexed by $\rho$, from the VGG-19 model \cite{vgg} pre-trained on ImageNet \cite{ImageNet}, and $W_{\rho}$,$H_{\rho }$,$C_{\rho}$ are the spatial width, height and depth of $\phi _{\rho }$, respectively. We found $\rho = Conv1\_ 2$ leads to the best results in our experiments. 
	
	The adversarial loss is derived from $D_{A}$ and $D_{S}$:
	
	\begin{small}
		\begin{equation}
		\begin{split}
		\mathcal{L}_{GAN}=&\mathbb{E}[\log [D_{A}(P_c,P_t) + (1-D_{A}(P_c,P_g)]]\\ 
		+&\mathbb{E}[\log [D_{S}(S_t,P_t) + (1-D_{S}(S_t,P_g))]].
		\end{split}
		\end{equation}
	\end{small}Note that $(P_c, P_t)$, $(S_c, S_t)$ and $P_g$ are in the distributions of real person images, real person poses and fake person images, respectively. 
	
	%\vspace{-2mm}
	\vspace{1ex}\noindent\textbf{Implementation details.}
	The implementation is built upon the popular Pytorch framework.
	Adam optimizer \cite{Kingma2014-Adam} is adopted to train the proposed model for around 90k iterations with $\beta_1=0.5,\beta_2=0.999$. Learning rate is initially set to $2\times 10^{-4}$, and linearly decay to 0 after 60k iterations. We use 4 PMTBs in the generator for both datasets. ($\alpha,\lambda_1$, $\lambda_2$) is set to (5, 1, 1). We use synchronized batch normalization~\cite{??} (SyncBN) in our full model for all datasets. We experimentally found SyncBN is beneficial to reduce ``hole'' artifacts. Dropout \cite{dropout} is only applied in the PMTBs, its rate set to 0.5. Leaky ReLU \cite{LeakyReLU} is applied after every convolution or normalization layers in the discriminators, and its negative slope coefficient is set to 0.2. Code is available at \url{https://github.com/tengteng95/Pose-Transfer}.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

